Numerical periodic normalization for codim 2 bifurcations of limit cycles with center manifold of dimension higher than 3

Explicit computational formulas for coefficients of the periodic normal forms of the three most complex codim 2 bifurcations of limit cycles with dimension of the center manifold equal to 4 or to 5 in generic autonomous ODEs are derived. The resulting formulas are independent of the dimension of the phase space and involve solutions of certain boundary-value problems as well as multilinear functions from the Taylor expansion of the ODE right-hand side near the cycle. The formulas allow one to distinguish between the complicated bifurcation scenarios which can happen near these codim 2 bifurcations of limit cycles, where 3-tori and 4-tori can be present. We apply our techniques to the study of a known laser model, a novel model from population biology, and one for mechanical vibrations; these models exhibit Limit Point--Neimark-Sacker, Period-Doubling--Neimark-Sacker and double Neimark-Sacker bifurcations. Lyapunov exponents are computed to numerically confirm the results of the normal form analysis, in particular with respect to the existence of stable invariant tori of various dimensions and chaos.

==> computation.tex <==
\section{Computation of critical coefficients}
\label{Section:Theory}
As was mentioned in the previous section, the stability of the extra torus appearing in the ``difficult" cases is determined by third 
order terms for the LPNS bifurcation and fifth order terms for the PDNS and NSNS bifurcations. 
In the ``simple" cases, second order derivatives are sufficient to determine the behaviour in the LPNS 
bifurcations and third order derivatives are sufficient in the PDNS and NSNS bifurcations. 
Therefore, we restrict our computations in this section to second order terms in the LPNS case and up 
to and including third order terms in the PDNS and NSNS cases. The expressions of the third order 
coefficients for { LPNS} and fourth and fifth order coefficients for PDNS and NSNS are 
given in Appendix C in \cite{lc2nf_arxiv}. Remark that for efficiency reasons these higher order coefficients 
are not computed in {\sc matcont}, unless explicitly requested by the user.

\subsection{LPNS}\label{Section:LPNS}

The four-dimensional critical center manifold $W^c(\Gamma)$ at
the LPNS bifurcation can be parametrized locally by
$(\xi_1,\xi_2,\tau) \in \R \times \C \times [0,T]$ as 
\begin{equation}
u=u_0(\tau)+\xi_1 v_1(\tau) + \xi_2 v_2(\tau) +\bar \xi_2 \bar v_2(\tau)+ H(\xi_1,\xi_2,\tau), 
\label{eq:CM_LPNS}
\end{equation}
where $H$ satisfies $H(\xi_1,\xi_2,T)=H(\xi_1,\xi_2,0)$ and has the Taylor expansion 
\begin{eqnarray}
 H(\xi_1,\xi_2,\tau)= \sum_{\substack{2\leq i+j+k\leq 3}} 
 \frac{1}{i!j!k!}h_{ijk}(\tau)\xi_1^i\xi_2^j\bar{\xi}_2^k + O(\|\xi\|^4) , \label{eq:H_LPNS}
\end{eqnarray}
where the eigenfunctions $v_1$ and $v_2$ are defined by 
\begin{eqnarray} \label{eq:EigenFunc_LPNS}
&&\left\{\begin{array}{rcl}
\dot{v}_1-A(\tau)v_1 - F(u_0) & = & 0,\ \tau \in [0,T], \\
v_1(T)-v_1(0) & = & 0,\\
\int_{0}^{T} {\langle v_1,F(u_0)\rangle d\tau} & = & 0,\\
\end{array}
\right. 
\end{eqnarray}
and
\begin{eqnarray}\label{eq:EigenFunc_LPNS_2}
&&\left\{\begin{array}{rcl}
\dot{v}_2-A(\tau)v_2+i\omega v_2 & = & 0,\ \tau \in [0,T], \\
v_2(T) - v_2(0) & = & 0,\\
\int_{0}^{T} {\langle v_2,v_2\rangle d\tau} - 1  & = & 0.\\
\end{array}
\right.
\end{eqnarray}

The functions $v_1$ and $v_2$ exist because of Lemma~2 of \cite{Io:88}. 
The functions $h_{ijk}$ will be found by solving appropriate
BVPs, assuming that \eqref{eq:P.1} restricted to $W^c(\Gamma)$ has
the normal form \eqref{eq:NF-LPNS}. 

The coefficients of the normal
form  arise from the solvability conditions for the BVPs as
integrals of scalar products over the interval $[0,T]$.
Specifically, those scalar products involve among other things the quadratic and
cubic terms of \eqref{eq:MULT} near the periodic solution $u_0$,
the generalized eigenfunction $v_1$ and eigenfunction $v_2$, and the
adjoint eigenfunctions $\varphi^*$, $v_1^*$ and $v_2^*$ as solutions
of the problems
\begin{eqnarray}
&&\left\{\begin{array}{rcl}
 \dot{\varphi}^*+A^{\rm T}(\tau)\varphi^* & = & 0,\ \tau \in [0,T], \\
 \varphi^*(T)-\varphi^*(0) & = & 0, \label{eq:AdjEigenFunc_LPNS}\\
 \int_{0}^{T} {\langle \varphi^*,v_1 \rangle d\tau} -1 & = & 0,
 \end{array} \right.
 \end{eqnarray}
 \begin{eqnarray}
 &&\left\{\begin{array}{rcl}
 \dot{v}_1^*+A^{\rm T}(\tau) v_1^*+\varphi^* & = & 0,\ \tau \in [0,T], \\
 v_1^*(T)-v_1^*(0) & = & 0, \label{eq:AdjEigenFunc_LPNS_2}\\
 \int_{0}^{T} {\langle v_1^*,v_1 \rangle d\tau} & = & 0,
 \end{array} \right. 
 \end{eqnarray}
and
 \begin{eqnarray}
 &&\left\{\begin{array}{rcl}
 \dot{v}_2^*+A^{\rm T}(\tau) v_2^*+i\omega v_2^* & = & 0,\ \tau \in [0,T], \\
 v_2^*(T)-v_2^*(0) & = & 0, \label{eq:AdjEigenFunc_LPNS_3}\\
 \int_{0}^{T} {\langle v_2^*,v_2\rangle d\tau} -1 & = & 0.
 \end{array} \right.
\end{eqnarray}

In what follows we will make use of the orthogonality condition
\begin{eqnarray}
\int_{0}^{T} {\langle \varphi^*,F(u_0) \rangle d\tau} = 0,
\label{orthLPNS}
\end{eqnarray}
and the normalization condition
\begin{eqnarray}
\int_{0}^{T} {\langle v_1^*,F(u_0) \rangle d\tau} = 1,
\label{normLPNS}
\end{eqnarray}
which can be easily obtained from \eqref{eq:EigenFunc_LPNS}, \eqref{eq:AdjEigenFunc_LPNS} 
and \eqref{eq:AdjEigenFunc_LPNS_2}.


To derive the normal form coefficients we write down the
homological equation and compare term by term. We therefore substitute (\ref{eq:CM_LPNS}) 
into (\ref{eq:P.1}), using (\ref{eq:MULT}), (\ref{eq:NF-LPNS}) and (\ref{eq:H_LPNS}). 
By collecting the constant and linear terms we get the identities
$$\dot{u}_0=F(u_0), \qquad \dot v_1-F(u_0)=A(\tau) v_1, \qquad \dot{v}_2+i\omega v_2=A(\tau) v_2,$$
and the complex conjugate of the last equation.

By collecting the $\xi_1^2$-terms we find an equation for $h_{200}$
\begin{equation}\label{eq:h200_LPNS}
 \dot h_{200}-A(\tau) h_{200}=B(\tau;v_1,v_1)-2 a_{200} v_1-2 \alpha_{200} \dot u_0+2 \dot v_1,
\end{equation}
to be solved in the space of functions satisfying
$h_{200}(T)=h_{200}(0)$. In this space, the differential operator
$\frac{d}{d\tau}-A(\tau)$ is singular and its null-space is
spanned by $\dot u_0$. The Fredholm solvability
condition
\[
 \int_0^{T} \langle \varphi^*,B(\tau;v_1,v_1)-2 a_{200} v_1-2 \alpha_{200} \dot u_0+
 2 \dot v_1 \rangle\; d \tau =0
\]
allows one to calculate the coefficient $a_{200}$ in (\ref{eq:NF-LPNS}) due to the required normalization 
in \eqref{eq:AdjEigenFunc_LPNS}, i.e.
\begin{equation} \label{eq:a200_LPNS}
 \boxed{a_{200}=\frac{1}{2}\int_0^{T} \langle \varphi^*,B(\tau;v_1,v_1)+2 A(\tau) v_1 \rangle\; d \tau,}
\end{equation}
taking \eqref{eq:EigenFunc_LPNS} and \eqref{orthLPNS} into account. With $a_{200}$ defined in this way, 
let $h_{200}$ be a solution of (\ref{eq:h200_LPNS}) in the space of functions satisfying $h_{200}(0)=h_{200}(T)$. Notice that if
$h_{200}$ is a solution of \eqref{eq:h200_LPNS}, then also $h_{200}+\varepsilon_1 F(u_0)$ satisfies
\eqref{eq:h200_LPNS}, since $F(u_0)$ is in the kernel of
the operator $\frac{d}{d\tau}-A(\tau)$. In order to obtain a unique solution (without a component along  the null
eigenspace) we impose the following orthogonality condition which determines the value of $\varepsilon_1$
$$ \int_0^{T} \langle v_1^*,h_{200}\rangle \; d\tau =0,$$
since \eqref{normLPNS} holds. Thus $h_{200}$ is the unique solution of the BVP
%
\begin{equation}  \label{eq:BVP_h200_LPNS}
\left\{\begin{array}{rcl}
\dot{h}_{200}-A(\tau) h_{200} - B(\tau;v_1,v_1) -2A(\tau)v_1+2 a_{200} v_1+2 \alpha_{200} 
\dot u_0-2\dot u_0 & = & 0,\ \tau \in [0,T], \\
h_{200}(T)- h_{200}(0) & = & 0,\\
\int_0^{T} \langle v_1^*,h_{200}\rangle \; d\tau & = & 0.
\end{array}
\right.
\end{equation}

By collecting the $\xi_2^2$-terms (or $\bar \xi_2^2$-terms) we find an equation for $h_{020}$
\begin{equation*}\label{eq:h020_LPNS}
 \dot h_{020}-A(\tau) h_{020}+2i\omega h_{020}=B(\tau;v_2,v_2),
\end{equation*}
(or its complex conjugate). This equation has a unique solution $h_{020}$ satisfying
$h_{020}(T)=h_{020}(0)$, since due to the spectral assumptions $e^{2i\omega T}$ is not a 
multiplier of the critical cycle. Thus, $h_{020}$ can be found by solving
\begin{equation}  \label{eq:BVP_h020_LPNS}
\left\{\begin{array}{rcl}
\dot h_{020}-A(\tau) h_{020}+2i\omega h_{020}-B(\tau;v_2,v_2) & = & 0,\ \tau \in [0,T], \\
h_{020}(T)- h_{020}(0) & = & 0.
\end{array}
\right.
\end{equation}

By collecting the $\xi_1\xi_2$-terms we obtain an equation for $h_{110}$
\begin{equation*}\label{eq:h110_LPNS}
\dot h_{110}-A(\tau) h_{110} + i\omega h_{110} = B(\tau;v_1,v_2)-b_{110}v_2 +\dot v_2+i\omega v_2,
\end{equation*}
to be solved in the space of functions satisfying $h_{110}(T)=h_{110}(0)$. In this space, the 
differential operator
$\frac{d}{d\tau}-A(\tau)+i\omega$ is singular, since $e^{i\omega T}$ is a critical multiplier. 
So we can impose the following Fredholm solvability condition
$$\int_0^{T} \langle v_2^*, B(\tau;v_1,v_2)-b_{110}v_2 +\dot v_2+i\omega v_2\rangle \; d\tau = 0,$$
which due to the normalization condition in \eqref{eq:AdjEigenFunc_LPNS_3} determines the value 
of the normal form coefficient $b_{110}$, yielding
\begin{equation} \label{eq:b110_LPNS}
 \boxed{b_{110}=\int_0^{T} \langle v_2^*,B(\tau;v_1,v_2)+ A(\tau) v_2 \rangle\; d \tau.}
\end{equation}
The nullspace belonging to the operator $\frac{d}{d\tau}-A(\tau)+i\omega$ is one-dimensional and 
spanned by $v_2$. To determine $h_{110}$ uniquely, we need to impose an orthogonality condition 
with a vector whose inproduct with $v_2$ is non-zero. $v_2^*$ can be choosen because of the 
normalisation condition in \eqref{eq:AdjEigenFunc_LPNS_3}. In fact, $h_{110}$ only appears in 
the normal form coefficient $b_{210}$ (see Appendix C.1 in \cite{lc2nf_arxiv}), and a different normalization 
of $h_{110}$ does not influence the value of that normal form coefficient. Therefore, we obtain 
$h_{110}$ as the unique solution of the BVP
\begin{equation}  \label{eq:BVP_h110_LPNS}
\left\{\begin{array}{rcl}
\dot h_{110}-A(\tau) h_{110} + i\omega h_{110} - B(\tau;v_1,v_2)+b_{110}v_2 -A(\tau) v_2& = & 0,\ 
\tau \in [0,T], \\
h_{110}(T)- h_{110}(0) & = & 0,\\
\int_0^{T} \langle v_2^*,h_{110}\rangle \; d\tau & = & 0.
\end{array}
\right.
\end{equation}

By collecting the $ \left|\xi_2\right|^2$-terms we obtain a singular equation for $h_{011}$, namely
\begin{equation*}\label{eq:h011_LPNS}
\dot h_{011}-A(\tau) h_{011} = B(\tau;v_2,\bar v_2)-a_{011}v_1-\alpha_{011}\dot u_0,
\end{equation*}
to be solved in the space of functions satisfying $h_{011}(T)=h_{011}(0)$. The non-trivial kernel 
of the operator
$\frac{d}{d\tau}-A(\tau)$ is spanned by $\dot u_0$. So, the following Fredholm solvability condition 
is involved
$$\int_0^{T} \langle \varphi^*,B(\tau;v_2,\bar v_2)-a_{011}v_1-\alpha_{011}\dot u_0\rangle \; d\tau = 0,$$
which gives us the expression for the normal form coefficient $a_{011}$, i.e.
\begin{equation} \label{eq:a011_LPNS}
 \boxed{a_{011}=\int_0^{T} \langle \varphi^*,B(\tau;v_2,\bar v_2) \rangle\; d \tau.}
\end{equation}
We impose the orthogonality condition with the adjoint generalized eigenfunction $v_1^*$ to obtain $h_{011}$ 
as the unique solution of 
\begin{equation}  \label{eq:BVP_h011_LPNS}
\left\{\begin{array}{rcl}
\dot h_{011}-A(\tau) h_{011} - B(\tau;v_2,\bar v_2)+a_{011}v_1+\alpha_{011}\dot u_0 & = & 0,\ \tau \in [0,T], \\
h_{011}(T)- h_{011}(0) & = & 0,\\
\int_0^{T} \langle v_1^*,h_{011}\rangle \; d\tau & = & 0.
\end{array}
\right.
\end{equation}

We remark that the values of $\alpha_{200}$ and $\alpha_{011}$ are not determined by the homological equation. 
We therefore put them equal to zero.

Third order coefficients are only needed to determine the stability of the torus, if this torus exists. 
For completeness, we have listed these terms in Appendix C in \cite{lc2nf_arxiv}.

\subsection{PDNS} \label{Section:PDNS}
The four-dimensional critical center manifold $W^c(\Gamma)$ at
the PDNS bifurcation can be parametrized locally by
$(\xi_1,\xi_2,\tau) \in \R \times \C \times [0,2T]$ as 
\begin{equation}
u=u_0(\tau)+\xi_1 v_1(\tau) + \xi_2 v_2(\tau) +\bar \xi_2 \bar v_2(\tau)+ H(\xi_1,\xi_2,\tau), \label{eq:CM_PDNS}
\end{equation}
where $H$ satisfies $H(\xi_1,\xi_2,2T)=H(\xi_1,\xi_2,0)$ and has the Taylor expansion 
\begin{equation}
 H(\xi_1,\xi_2,\tau)= \sum_{2\leq i+j+k\leq 5} \frac{1}{i!j!k!}h_{ijk}(\tau)
 \xi_1^i\xi_2^j\bar{\xi}_2^k
+ O(\|\xi\|^6) , 
\label{eq:H_PDNS}
\end{equation}
while the eigenfunctions $v_1$ and $v_2$ are defined by 
\begin{eqnarray} \label{eq:EigenFunc_PDNS}
&&\left\{\begin{array}{rcl}
\dot{v}_1-A(\tau)v_1 & = & 0,\ \tau \in [0,T], \\
v_1(T)+v_1(0) & = & 0,\\
\int_{0}^{T} {\langle v_1,v_1\rangle d\tau} -1 & = & 0,\\
\end{array}
\right. 
\end{eqnarray}
with $v_1(\tau+T)=-v_1(\tau)$ for $\tau \in [0,T]$ and
\begin{eqnarray}\label{eq:EigenFunc_PDNS_2}
&&\left\{\begin{array}{rcl}
\dot{v}_2-A(\tau)v_2+i\omega v_2 & = & 0,\ \tau \in [0,T], \\
v_2(T) - v_2(0) & = & 0,\\
\int_{0}^{T} {\langle v_2,v_2\rangle d\tau} - 1  & = & 0.\\
\end{array}
\right.
\end{eqnarray}

The functions $v_1$ and $v_2$ exist because of Lemma~5 of \cite{Io:88}. 
The functions $h_{ijk}$ can be found by solving appropriate
BVPs, assuming that \eqref{eq:P.1} restricted to $W^c(\Gamma)$ has
the normal form \eqref{eq:NF-PDNS}. Moreover, $u(\tau,\xi_1,\xi_2,\bar\xi_2) = 
u(\tau+T,-\xi_1,\xi_2,\bar\xi_2)$ so that
\begin{equation}
h_{ijk}(\tau)= (-1)^ih_{ijk}(\tau+T),
\label{propertyhijk}
\end{equation}
for $\tau \in [0,T]$. Therefore, we can restrict our computations to the interval $[0,T]$ instead of $[0,2T]$.

The coefficients of the normal
form  arise from the solvability conditions for the BVPs as
integrals of scalar products over the interval $[0,T]$.
Specifically, those scalar products involve among other things the quadratic and
cubic terms of \eqref{eq:MULT} near the periodic solution $u_0$,
$v_1$, $v_2$, and the
adjoint eigenfunctions $\varphi^*$, $v_1^*$ and $v_2^*$ as solutions
of the problems
\begin{eqnarray}
&&\left\{\begin{array}{rcl}
 \dot{\varphi}^*+A^{\rm T}(\tau)\varphi^* & = & 0,\ \tau \in [0,T], \\
 \varphi^*(T)-\varphi^*(0) & = & 0, \label{eq:AdjEigenFunc_PDNS}\\
 \int_{0}^{T} {\langle \varphi^*,F(u_0) \rangle d\tau} -1 & = & 0,
 \end{array} \right.
 \end{eqnarray}
 \begin{eqnarray}
 &&\left\{\begin{array}{rcl}
 \dot{v}_1^*+A^{\rm T}(\tau) v_1^* & = & 0,\ \tau \in [0,T], \\
 v_1^*(T)+v_1^*(0) & = & 0, \label{eq:AdjEigenFunc_PDNS_2}\\
 \int_{0}^{T} {\langle v_1^*,v_1 \rangle d\tau} -1& = & 0,
 \end{array} \right. 
 \end{eqnarray}
and
 \begin{eqnarray}
 &&\left\{\begin{array}{rcl}
 \dot{v}_2^*+A^{\rm T}(\tau) v_2^*+i\omega v_2^* & = & 0,\ \tau \in [0,T], \\
 v_2^*(T)-v_2^*(0) & = & 0, \label{eq:AdjEigenFunc_PDNS_3}\\
 \int_{0}^{T} {\langle v_2^*,v_2\rangle d\tau} -1 & = & 0.
 \end{array} \right.
\end{eqnarray}

By collecting the constant and linear terms we get the identities
$$
 \dot{u}_0=F(u_0), \qquad \dot v_1=A(\tau) v_1, \qquad \dot{v}_2+i\omega v_2=A(\tau) v_2,
$$
and the complex conjugate of the last equation, which merely reflect the definition of $u_0$ and (\ref{eq:EigenFunc_PDNS}), (\ref{eq:EigenFunc_PDNS_2}).

By collecting the $\xi_1^2$-terms we find an equation for $h_{200}$
\begin{equation}\label{eq:h200_PDNS}
 \dot h_{200}-A(\tau) h_{200}=B(\tau;v_1,v_1)-2 \alpha_{200} \dot u_0,
\end{equation}
to be solved in the space of functions satisfying
$h_{200}(T)=h_{200}(0)$. In this space, the differential operator
$\frac{d}{d\tau}-A(\tau)$ is singular and its null-space is
spanned by $\dot u_0$. The Fredholm solvability
condition
\[
 \int_0^{T} \langle \varphi^*,B(\tau;v_1,v_1)-2 \alpha_{200} \dot u_0 \rangle\; d \tau =0
\]
gives us the possibility to calculate $\alpha_{200}$ in (\ref{eq:NF-LPNS}) by the required normalization in \eqref{eq:AdjEigenFunc_PDNS}, i.e.
\begin{equation} \label{eq:alpha200_PDNS}
 \alpha_{200}=\frac{1}{2}\int_0^{T} \langle \varphi^*,B(\tau;v_1,v_1) \rangle\; d \tau.
\end{equation}
As before, $h_{200}$ is determined up to the addition of a multiple of $\dot u_0$, since $h_{200}+\varepsilon_1 F(u_0)$ is a solution of \eqref{eq:h200_PDNS} for every value of $\varepsilon_1$. We fix the value of $h_{200}$ by demanding the orthogonality with the adjoint eigenfunction corresponding with multiplier $1$, i.e.
$$ \int_0^{T} \langle \varphi^*,h_{200}\rangle \; d\tau =0.$$
We obtain $h_{200}$ then as the unique solution of the BVP
\begin{equation}  \label{eq:BVP_h200_PDNS}
\left\{\begin{array}{rcl}
\dot{h}_{200}-A(\tau) h_{200} -B(\tau;v_1,v_1)+2 \alpha_{200} \dot u_0& = & 0,\ \tau \in [0,T], \\
h_{200}(T)- h_{200}(0) & = & 0,\\
\int_0^{T} \langle \varphi^*,h_{200}\rangle \; d\tau & = & 0.
\end{array}
\right.
\end{equation}

By collecting the $\xi_2^2$-terms (or $\bar \xi_2^2$-terms) we find the differential equation for $h_{020}$
\begin{equation*}\label{eq:h020_PDNS}
 \dot h_{020}-A(\tau) h_{020}+2i\omega h_{020}=B(\tau;v_2,v_2),
\end{equation*}
or its complex conjugate. Since $e^{2i\omega T}$ is not a critical multiplier, no Fredholm solvability condition has to be satisified. $h_{020}$ can thus simply be found by solving
\begin{equation}  \label{eq:BVP_h020_PDNS}
\left\{\begin{array}{rcl}
\dot h_{020}-A(\tau) h_{020}+2i\omega h_{020}-B(\tau;v_2,v_2) & = & 0,\ \tau \in [0,T], \\
h_{020}(T)- h_{020}(0) & = & 0.
\end{array}
\right.
\end{equation}

The equation found by comparing the $\xi_1\xi_2$-terms is given by
\begin{equation*}\label{eq:h110_PDNS}
\dot h_{110}-A(\tau) h_{110} + i\omega h_{110} = B(\tau;v_1,v_2).
\end{equation*}
From \eqref{propertyhijk} it follows that $h_{110}$ is anti-periodic. Now, since $-e^{i\omega T}$ is not a multiplier of the critical cycle, no solvability condition has to be satisfied. Therefore, we can immediately obtain $h_{110}$ from 
\begin{equation}  \label{eq:BVP_h110_PDNS}
\left\{\begin{array}{rcl}
\dot h_{110}-A(\tau) h_{110} + i\omega h_{110} - B(\tau;v_1,v_2)& = & 0,\ \tau \in [0,T], \\
h_{110}(T)+ h_{110}(0) & = & 0,\\
\end{array}
\right.
\end{equation}

The $\left|\xi_2\right|^2$-terms lead to a singular equation for $h_{011}$, namely
\begin{equation*}\label{eq:h011_PDNS}
\dot h_{011}-A(\tau) h_{011} = B(\tau;v_2,\bar v_2)-\alpha_{011}\dot u_0,
\end{equation*}
to be solved in the space of $T$-periodic functions. The non-trivial kernel of the operator
$\frac{d}{d\tau}-A(\tau)$ is spanned by $\dot u_0$. So, the Fredholm solvability condition with the corresponding $T$-periodic adjoint eigenfunction is involved, i.e.
$$\int_0^{T} \langle \varphi^*,B(\tau;v_2,\bar v_2)-\alpha_{011}\dot u_0\rangle \; d\tau = 0,$$
from which the expression for the normal form coefficient $\alpha_{011}$ can be derived
\begin{equation} \label{eq:alpha011_PDNS}
 \alpha_{011}=\int_0^{T} \langle \varphi^*,B(\tau;v_2,\bar v_2) \rangle\; d \tau.
\end{equation}
Now, we still need to uniquely determine the multiple of $F(u_0)$ which can be added to the function $h_{011}$, and will therefore impose the orthogonality condition with $\varphi^*$ to obtain $h_{011}$ as the unique solution of 
\begin{equation}  \label{eq:BVP_h011_PDNS}
\left\{\begin{array}{rcl}
\dot h_{011}-A(\tau) h_{011} - B(\tau;v_2,\bar v_2)+\alpha_{011}\dot u_0 & = & 0,\ \tau \in [0,T], \\
h_{011}(T)- h_{011}(0) & = & 0,\\
\int_0^{T} \langle \varphi^*,h_{011}\rangle \; d\tau & = & 0.
\end{array}
\right.
\end{equation}
We have now examined all order two terms, and continue with the order three terms. 

Collecting the $\xi_1^3$-terms gives an equation for $h_{300}$ and will give us the possibility to compute the normal form coefficient $a_{300}$ in \eqref{eq:NF-PDNS}. The differential equation
\begin{equation*}\label{eq:h300_PDNS}
 \dot h_{300}-A(\tau) h_{300}=C(\tau;v_1,v_1,v_1)+3B(\tau;v_1,h_{200})-6 \alpha_{200} \dot v_1-6a_{300}v_1
\end{equation*}
has to be solved in the space of functions satisfying $h_{300}(T)=-h_{300}(0)$. The non-trivial anti-periodic kernel of the operator
$\frac{d}{d\tau}-A(\tau)$ is spanned by $v_1$. So, the Fredholm solvability condition with the anti-periodic adjoint eigenfunction $v_1^*$ is involved, i.e.
$$\int_0^{T} \langle v_1^*,C(\tau;v_1,v_1,v_1)+3B(\tau;v_1,h_{200})-6 \alpha_{200} \dot v_1-6a_{300}v_1\rangle \; d\tau = 0$$
and thus
\begin{equation} \label{eq:a300_PDNS}
 \boxed{a_{300}= \frac{1}{6} \int_0^{T} \langle v_1^*,C(\tau;v_1,v_1,v_1)+3B(\tau;v_1,h_{200})-6 \alpha_{200} A(\tau)v_1 \rangle\; d \tau,}
\end{equation}
due to the normalization condition from \eqref{eq:AdjEigenFunc_PDNS_2}. 
The usual orthogonality condition with the adjoint eigenfunction $v_1^*$ is imposed to obtain $h_{300}$ as the unique solution of 
\begin{equation}  \label{eq:BVP_h300_PDNS}
\left\{\begin{array}{rcl}
\dot h_{300}-A(\tau) h_{300}-C(\tau;v_1,v_1,v_1)-3B(\tau;v_1,h_{200})\\
+6 \alpha_{200} A(\tau) v_1+6a_{300}v_1 & = & 0,\ \tau \in [0,T], \\
h_{300}(T)+ h_{300}(0) & = & 0,\\
\int_0^{T} \langle v_1^*,h_{300}\rangle \; d\tau & = & 0.
\end{array}
\right.
\end{equation}

The $\xi_2^3$ (or $\bar \xi_2^3$)-terms from the homological equation give an equation for $h_{030}$
\begin{equation*}\label{eq:h030_PDNS}
 \dot h_{030}-A(\tau) h_{030}+3i\omega h_{030}=C(\tau;v_2,v_2,v_2)+3B(\tau;v_2,h_{020}),
\end{equation*}
or its complex conjugate. This equation has a unique solution $h_{030}$ satisfying
$h_{030}(T)=h_{030}(0)$, since due to the spectral assumptions $e^{3i\omega T}$ is not a multiplier of the critical cycle. Thus, $h_{030}$ can be found by solving
\begin{equation}  \label{eq:BVP_h030_PDNS}
\left\{\begin{array}{rcl}
\dot h_{030}-A(\tau) h_{030}+3i\omega h_{030}-C(\tau;v_2,v_2,v_2)-3B(\tau;v_2,h_{020}) & = & 0,\ \tau \in [0,T], \\
h_{030}(T)- h_{030}(0) & = & 0.
\end{array}
\right.
\end{equation}

By collecting the $\xi_1^2\xi_2$-terms we find an equation for $h_{210}$
\begin{equation}\label{eq:h210_PDNS}
\begin{array}{rcl}
 \dot h_{210}-A(\tau) h_{210}+i\omega h_{210}&=&C(\tau;v_1,v_1,v_2)+B(\tau;v_2,h_{200})+2B(\tau;v_1,h_{110})\\
 &-&2 \alpha_{200} \dot v_2-2b_{210}v_2-2i\omega \alpha_{200}v_2,
\end{array}
\end{equation}
to be solved in the space of $T$-periodic functions. The non-trivial kernel of the operator
$\frac{d}{d\tau}-A(\tau)+i\omega$ is spanned by the complex eigenfunction $v_2$. So, the following Fredholm solvability condition has to be imposed
\begin{eqnarray*}
\int_0^{T} \langle v_2^*,C(\tau;v_1,v_1,v_2)+B(\tau;v_2,h_{200})+2B(\tau;v_1,h_{110})\\ 
-2 \alpha_{200} \dot v_2-2b_{210}v_2-2i\omega \alpha_{200}v_2\rangle \; d\tau &=& 0.
\end{eqnarray*}
From this, the expression for the normal form coefficient $b_{210}$ can be derived, namely
\begin{equation} \label{eq:b210_PDNS}
 \boxed{b_{210}=\frac{1}{2}\!\int_0^{T}\! \langle v_2^*,C(\tau;v_1,v_1,v_2)+B(\tau;v_2,h_{200})+2B(\tau;v_1,h_{110})-2 \alpha_{200} A(\tau) v_2 \rangle d \tau,}
\end{equation}
taking the normalization from \eqref{eq:AdjEigenFunc_PDNS_3} into account. Now, $h_{210}$ is defined by \eqref{eq:h210_PDNS} up to a multiple of $v_2$, therefore we impose the orthogonality condition with the adjoint eigenfunction $v_2^*$ to obtain $h_{210}$ as the unique solution of 
\begin{equation}  \label{eq:BVP_h210_PDNS}
\left\{\begin{array}{rcl}
\dot h_{210}-A(\tau) h_{210}+i\omega h_{210}-C(\tau;v_1,v_1,v_2)-B(\tau;v_2,h_{200})\\
-2B(\tau;v_1,h_{110})+2 \alpha_{200} A(\tau) v_2+2b_{210}v_2 & = & 0,\ \tau \in [0,T], \\
h_{210}(T)- h_{210}(0) & = & 0,\\
\int_0^{T} \langle v_2^*,h_{210}\rangle \; d\tau & = & 0.
\end{array}
\right.
\end{equation}

Since $\xi_1\xi_2^2$ is not a term in the normal form \eqref{eq:NF-PDNS}, we will find a non-singular equation for $h_{120}$ when collecting the $\xi_1\xi_2^2$-terms from the homological equation. Moreover, because of property \eqref{propertyhijk} $h_{120}$ is anti-periodic and thus 
\begin{equation}  \label{eq:BVP_h120_PDNS}
\left\{\begin{array}{rcl}
\dot h_{120}-A(\tau) h_{120}+2i\omega h_{120}-C(\tau;v_1,v_2,v_2)\\
-B(\tau;v_1,h_{020})-2B(\tau;v_2,h_{110}) & = & 0,\ \tau \in [0,T], \\
h_{120}(T)+ h_{120}(0) & = & 0.
\end{array}
\right.
\end{equation}

The two remaining third order terms are the $\xi_2\left|\xi_2\right|^2$-terms and the 
$\xi_1\left|\xi_2\right|^2$-terms, which both give a singular equation, namely
\begin{eqnarray*}\label{eq:h021_PDNS}
 \dot h_{021}-A(\tau) h_{021}+i\omega h_{021}&=&C(\tau;v_2,v_2,\bar v_2)+B(\tau;\bar v_2,h_{020})+
 2B(\tau;v_2,h_{011})\\
 &-&2 \alpha_{011} \dot v_2-2b_{021}v_2-2i\omega\alpha_{011}v_2
\end{eqnarray*}
and 
\begin{eqnarray*}\label{eq:h111_PDNS}
 \dot h_{111}-A(\tau) h_{111}&=&C(\tau;v_1,v_2,\bar v_2)+B(\tau;v_1,h_{011})+B(\tau;v_2,h_{101})+
 B(\tau;\bar v_2,h_{110})\\
 &-& \alpha_{011} \dot v_1-a_{111}v_1.
\end{eqnarray*}
The first function is $T$-periodic, the second one is anti-periodic. Both involve a Fredholm solvability condition, which leads to the computation of the two remaining unknown third order normal form coefficients of \eqref{eq:NF-PDNS}, i.e.
\begin{equation} \label{eq:b021_PDNS}
 \boxed{b_{021}=\frac{1}{2} \int_0^{T} \langle v_2^*,C(\tau;v_2,v_2,\bar v_2)+B(\tau;\bar v_2,h_{020})+2B(\tau;v_2,h_{011})-2 \alpha_{011} A(\tau) v_2 \rangle\; d \tau}
\end{equation}
and 
\begin{equation} \label{eq:a111_PDNS}
 \boxed{a_{111}= \int_0^{T} \langle v_1^*,C(\tau;v_1,v_2,\bar v_2)+B(\tau;v_1,h_{011})+2\Re(B(\tau;v_2,h_{101}))- \alpha_{011}A(\tau)v_1\rangle\; d \tau.}
\end{equation}
Since we need both $h_{021}$ and $h_{111}$ for the computation of higher order normal form coefficients, we also write 
down their BVPs
\begin{equation}  \label{eq:BVP_h021_PDNS}
\left\{\begin{array}{rcl}
\dot h_{021}-A(\tau) h_{021}+i\omega h_{021}-C(\tau;v_2,v_2,\bar v_2)-B(\tau;\bar v_2,h_{020})\\
-2B(\tau;v_2,h_{011})+2 \alpha_{011} A(\tau) v_2+2b_{021}v_2 & = & 0,\ \tau \in [0,T], \\
h_{021}(T)- h_{021}(0) & = & 0,\\
\int_0^{T} \langle v_2^*,h_{021}\rangle \; d\tau & = & 0
\end{array}
\right.
\end{equation}
and 
\begin{equation}  \label{eq:BVP_h111_PDNS}
\left\{\begin{array}{rcl}
\dot h_{111}-A(\tau) h_{111}-C(\tau;v_1,v_2,\bar v_2)-B(\tau;v_1,h_{011})\\
-2\Re(B(\tau;v_2,h_{101}))+\alpha_{011} A(\tau) v_1+a_{111}v_1 & = & 0,\ \tau \in [0,T], \\
h_{111}(T)+ h_{111}(0) & = & 0,\\
\int_0^{T} \langle v_1^*,h_{111}\rangle \; d\tau & = & 0.
\end{array}
\right.
\end{equation}

The stability of a possibly existing torus depends on the fourth and fifth order coefficients, which we have listed in Appendix C in \cite{lc2nf_arxiv}.

\subsection{NSNS}\label{Section:NSNS}
The five-dimensional critical center manifold $W^c(\Gamma)$ at
the NSNS bifurcation can be parametrized locally by
$(\xi,\tau) \in \C^2 \times [0,T]$ as 
\begin{equation}
u=u_0(\tau)+\xi_1 v_1(\tau)+\bar \xi_1 \bar v_1(\tau) + \xi_2 v_2(\tau) +\bar \xi_2 \bar v_2(\tau)+ 
H(\xi,\tau), \label{eq:CM_NSNS}
\end{equation}
%%
where $H$ satisfies $H(\xi,T)=H(\xi,0)$ and has the Taylor
expansion %%
\begin{equation}
 H(\xi,\tau)= \sum_{2\leq i+j+k+l\leq 5} \frac{1}{i!j!k!l!}h_{ijkl}(\tau)
 \xi_1^i\bar{\xi}_1^j\xi_2^k\bar{\xi}_2^l + O(\|\xi\|^6) , 
\label{eq:H_NSNS}
\end{equation}
where the complex eigenfunctions $v_1$ and $v_2$ are given by 
\begin{eqnarray} \label{eq:EigenFunc_NSNS}
&&\left\{\begin{array}{rcl}
\dot{v}_1-A(\tau)v_1 +i\omega_1 v_1 & = & 0,\ \tau \in [0,T], \\
v_1(T)-v_1(0) & = & 0,\\
\int_{0}^{T} {\langle v_1,v_1\rangle d\tau}-1 & = & 0,\\
\end{array}
\right. 
\end{eqnarray}
and
\begin{eqnarray}\label{eq:EigenFunc_NSNS_2}
&&\left\{\begin{array}{rcl}
\dot{v}_2-A(\tau)v_2+i\omega_2 v_2 & = & 0,\ \tau \in [0,T], \\
v_2(T) - v_2(0) & = & 0,\\
\int_{0}^{T} {\langle v_2,v_2\rangle d\tau} - 1  & = & 0.\\
\end{array}
\right.
\end{eqnarray}

The functions $v_1$ and $v_2$ exist because of Lemma~2 of \cite{Io:88}. %%
The functions $h_{ijkl}$ will be found by solving appropriate
BVPs, assuming that \eqref{eq:P.1} restricted to $W^c(\Gamma)$ has
the normal form \eqref{eq:NF-NSNS}. 

The coefficients of the normal
form  arise from the solvability conditions for the BVPs as
integrals of scalar products over the interval $[0,T]$.
Specifically, those scalar products involve among other things the quadratic and
cubic terms of \eqref{eq:MULT} near the periodic solution $u_0$,
the eigenfunctions $v_1$ and $v_2$, and the
adjoint eigenfunctions $\varphi^*$, $v_1^*$ and $v_2^*$ as solution
of the problems
\begin{eqnarray}
&&\left\{\begin{array}{rcl}
 \dot{\varphi}^*+A^{\rm T}(\tau)\varphi^* & = & 0,\ \tau \in [0,T], \\
 \varphi^*(T)-\varphi^*(0) & = & 0, \label{eq:AdjEigenFunc_NSNS}\\
 \int_{0}^{T} {\langle \varphi^*,F(u_0) \rangle d\tau} -1 & = & 0,
 \end{array} \right.
 \end{eqnarray}
 \begin{eqnarray}
 &&\left\{\begin{array}{rcl}
 \dot{v}_1^*+A^{\rm T}(\tau) v_1^*+i\omega_1v_1^* & = & 0,\ \tau \in [0,T], \\
 v_1^*(T)-v_1^*(0) & = & 0, \label{eq:AdjEigenFunc_NSNS_2}\\
 \int_{0}^{T} {\langle v_1^*,v_1 \rangle d\tau}-1 & = & 0,
 \end{array} \right. 
 \end{eqnarray}
and
 \begin{eqnarray}
 &&\left\{\begin{array}{rcl}
 \dot{v}_2^*+A^{\rm T}(\tau) v_2^*+i\omega_2 v_2^* & = & 0,\ \tau \in [0,T], \\
 v_2^*(T)-v_2^*(0) & = & 0, \label{eq:AdjEigenFunc_NSNS_3}\\
 \int_{0}^{T} {\langle v_2^*,v_2\rangle d\tau} -1 & = & 0.
 \end{array} \right.
\end{eqnarray}


By collecting the constant and linear terms we get the identities
\begin{eqnarray}
 \dot{u}_0=F(u_0), \qquad \dot v_1+ i\omega_1 v_1=A(\tau) v_1, \qquad \dot{v}_2+i\omega_2 v_2=A(\tau) v_2,
\label{basiceqnsns}
\end{eqnarray}
and the complex conjugates of the last two equations. (\ref{basiceqnsns}) merely reflects the definition of $u_0$ and the first equations in \eqref{eq:EigenFunc_NSNS}, \eqref{eq:EigenFunc_NSNS_2}.

By collecting the $\xi_1^2$ (or $\bar \xi_1^2$-terms)-terms we find an equation for $h_{2000}$
\begin{equation*}\label{eq:h2000_NSNS}
 \dot h_{2000}-A(\tau) h_{2000}+2i\omega_1h_{2000}=B(\tau;v_1,v_1),
\end{equation*}
(or its complex conjugate). This equation has a unique solution $h_{2000}$ satisfying
$h_{2000}(T)=h_{2000}(0)$, since due to the spectral assumptions $e^{2i\omega_1 T}$ is not a multiplier of the critical cycle. Thus, $h_{2000}$ can be found by solving
\begin{equation}  \label{eq:BVP_h2000_NSNS}
\left\{\begin{array}{rcl}
\dot h_{2000}-A(\tau) h_{2000}+2i\omega_1h_{2000}-B(\tau;v_1,v_1) & = & 0,\ \tau \in [0,T], \\
h_{2000}(T)- h_{2000}(0) & = & 0.
\end{array}
\right.
\end{equation}
The function $h_{0200}$ is just the complex conjugate of the function $h_{2000}$. Analogously, by comparing the $\xi_2^2$-terms, we find that $h_{0020}$ is the unique solution of 
\begin{equation}  \label{eq:BVP_h0020_NSNS}
\left\{\begin{array}{rcl}
\dot h_{0020}-A(\tau) h_{0020}+2i\omega_2h_{0020}-B(\tau;v_2,v_2) & = & 0,\ \tau \in [0,T], \\
h_{0020}(T)- h_{0020}(0) & = & 0.
\end{array}
\right.
\end{equation}

By collecting the $\left|\xi_1\right|^2$-terms we obtain a singular equation, as expected since this term is present in the normal form \eqref{eq:NF-NSNS}, namely
\begin{equation*}\label{eq:h1100_NSNS}
 \dot h_{1100}-A(\tau) h_{1100}=B(\tau;v_1,\bar v_1)-\alpha_{1100}\dot u_0,
\end{equation*}
to be solved in the space of functions satisfying
$h_{1100}(T)=h_{1100}(0)$. Since the null-space is
spanned by $\dot u_0$, the Fredholm solvability
condition
\[
 \int_0^{T} \langle \varphi^*,B(\tau;v_1,\bar v_1)-\alpha_{1100}\dot u_0 \rangle\; d \tau =0
\]
gives us the possibility to calculate parameter $\alpha_{1100}$ due to the normalization condition in \eqref{eq:AdjEigenFunc_NSNS}, i.e.
\begin{equation} \label{eq:alpha1100_NSNS}
 \alpha_{1100}=\int_0^{T} \langle \varphi^*,B(\tau;v_1,\bar v_1)\rangle\; d \tau.
\end{equation}
Function $h_{1100}$ is now determined up to the addition of a multiple of $\dot u_0$. As always, we will add an orthogonality condition, in this case with the adjoint eigenfunction coresponding with multiplier $1$. Therefore, with the value of $\alpha_{1100}$ from \eqref{eq:alpha1100_NSNS} we obtain $h_{1100}$ as the unique solution of the BVP
\begin{equation}  \label{eq:BVP_h1100_NSNS}
\left\{\begin{array}{rcl}
\dot{h}_{1100}-A(\tau) h_{1100} - B(\tau;v_1,\bar v_1) + \alpha_{1100} \dot u_0 & = & 0,\ \tau \in [0,T], \\
h_{1100}(T)- h_{1100}(0) & = & 0,\\
\int_0^{T} \langle \varphi^*,h_{1100}\rangle \; d\tau & = & 0.
\end{array}
\right.
\end{equation}

Analogously, function $h_{0011}$ can be obtained by solving
\begin{equation}  \label{eq:BVP_h0011_NSNS}
\left\{\begin{array}{rcl}
\dot{h}_{0011}-A(\tau) h_{0011} - B(\tau;v_2,\bar v_2) + \alpha_{0011} \dot u_0 & = & 0,\ \tau \in [0,T], \\
h_{0011}(T)- h_{0011}(0) & = & 0,\\
\int_0^{T} \langle \varphi^*,h_{0011}\rangle \; d\tau & = & 0,
\end{array}
\right.
\end{equation}
with 
\begin{equation} \label{eq:alpha0011_NSNS}
 \alpha_{0011}=\int_0^{T} \langle \varphi^*,B(\tau;v_2,\bar v_2)\rangle\; d \tau.
\end{equation}

By collecting the $\xi_1\xi_2$-terms we find the following differential equation for $h_{1010}$
\begin{equation*}\label{eq:h1010_NSNS}
 \dot h_{1010}-A(\tau) h_{1010}+i\omega_1 h_{1010}+i\omega_2 h_{1010}=B(\tau;v_1,v_2).
\end{equation*}
This equation has a unique solution $h_{1010}$ satisfying
$h_{1010}(T)=h_{1010}(0)$, since due to the spectral assumptions $e^{i(\omega_1+\omega_2) T}$ is not a multiplier of the critical cycle. Thus, $h_{1010}$ can be found by solving
\begin{equation}  \label{eq:BVP_h1010_NSNS}
\left\{\begin{array}{rcl}
\dot h_{1010}-A(\tau) h_{1010}+i\omega_1 h_{1010}+i\omega_2 h_{1010}-B(\tau;v_1,v_2) & = & 0,\ \tau \in [0,T], \\
h_{1010}(T)- h_{1010}(0) & = & 0.
\end{array}\right.
\end{equation}
We note that $h_{0101} = \overline{h_{1010}}$.

The last second order derivative coming from looking at the $\xi_1\bar \xi_2$-terms results in a non-singular differential equation, such that 
\begin{equation}  \label{eq:BVP_h1001_NSNS}
\left\{\begin{array}{rcl}
\dot h_{1001}-A(\tau) h_{1001}+i\omega_1 h_{1001}-i\omega_2 h_{1001}-B(\tau;v_1,\bar v_2) & = & 0,\ \tau \in [0,T], \\
h_{1001}(T)- h_{1001}(0) & = & 0.
\end{array}\right.
\end{equation}

We now come to the third order terms. From the $\xi_1^3$ and $\xi_2^3$-terms we immediately get the BVPs for $h_{3000}$ and $h_{0030}$, namely
\begin{equation}  \label{eq:BVP_h3000_NSNS}
\left\{\begin{array}{rcl}
 \dot h_{3000}-A(\tau) h_{3000}+3i\omega_1 h_{3000}-C(\tau;v_1,v_1,v_1)\\
-3B(\tau;v_1,h_{2000}) & = & 0,\ \tau \in [0,T], \\
h_{3000}(T)- h_{3000}(0) & = & 0
\end{array}\right.
\end{equation}
and 
\begin{equation}  \label{eq:BVP_h0030_NSNS}
\left\{\begin{array}{rcl}
 \dot h_{0030}-A(\tau) h_{0030}+3i\omega_2 h_{0030}-C(\tau;v_2,v_2,v_2)\\
-3B(\tau;v_2,h_{0020}) & = & 0,\ \tau \in [0,T], \\
h_{0030}(T)- h_{0030}(0) & = & 0.
\end{array}\right.
\end{equation}

Since the $\xi_1\left|\xi_1\right|^2$-term is present in the normal form for the double Neimark-Sacker bifurcation, a Fredholm solvability condition is involved coming from the following differential equation for $h_{2100}$
\begin{eqnarray*}
 \dot h_{2100}-A(\tau) h_{2100}+i\omega_1 h_{2100}&=&C(\tau;v_1,v_1,\bar v_1)+2B(\tau;v_1,h_{1100})+B(\tau;\bar v_1,h_{2000})\nonumber\\
 &&-2a_{2100}v_1-2i\omega_1\alpha_{1100}v_1-2\alpha_{1100} \dot v_1.\nonumber\\\label{eq:h2100_NSNS}
\end{eqnarray*}
The differential operator
$\frac{d}{d\tau}-A(\tau)+i\omega_1$ is singular with its null-space
spanned by $v_1$, so we get
condition
\begin{eqnarray*}
 \int_0^{T} \langle v_1^*,C(\tau;v_1,v_1,\bar v_1)+2B(\tau;v_1,h_{1100})+B(\tau;\bar v_1,h_{2000})-2a_{2100}v_1 && \\
 -2\alpha_{1100} \dot v_1 -2i\omega_1\alpha_{1100}v_1\rangle\; d \tau &=& 0.
 \end{eqnarray*}
Taking the normalization condition from \eqref{eq:AdjEigenFunc_NSNS_2} and the differential equation from \eqref{eq:EigenFunc_NSNS} into account, we get
\begin{equation} \label{eq:a2100_NSNS}
 \boxed{a_{2100}=\frac{1}{2} \int_0^{T} \langle v_1^*,C(\tau;v_1,v_1,\bar v_1)+2B(\tau;v_1,h_{1100})+B(\tau;\bar v_1,h_{2000})-2\alpha_{1100} A(\tau) v_1\rangle\; d \tau.}
\end{equation}
Therefore, we can compute $h_{2100}$ as the unique solution of the BVP
\begin{equation}  \label{eq:BVP_h2100_NSNS}
\left\{\begin{array}{rcl}
\dot h_{2100}-A(\tau) h_{2100}+i\omega_1 h_{2100}-C(\tau;v_1,v_1,\bar v_1)\\
-2B(\tau;v_1,h_{1100})-B(\tau;\bar v_1,h_{2000})+2a_{2100}v_1+2\alpha_{1100}A(\tau) v_1& = & 0,\ \tau \in [0,T], \\
h_{2100}(T)- h_{2100}(0) & = & 0,\\
\int_0^{T} \langle v_1^*,h_{2100}\rangle \; d\tau & = & 0.
\end{array}
\right.
\end{equation}

We can now immediately list the following four BVPs
\begin{equation}  \label{eq:BVP_h2010_NSNS}
\left\{\begin{array}{rcl}
 \dot h_{2010}-A(\tau) h_{2010}+2i\omega_1 h_{2010}+i\omega_2 h_{2010}-C(\tau;v_1,v_1,v_2)&&\\
 -B(\tau;v_2,h_{2000})-2B(\tau;v_1,h_{1010})& = & 0,\ \tau \in [0,T], \\
h_{2010}(T)- h_{2010}(0) & = & 0,
\end{array}\right.
\end{equation}
\begin{equation}  \label{eq:BVP_h2001_NSNS}
\left\{\begin{array}{rcl}
 \dot h_{2001}-A(\tau) h_{2001}+2i\omega_1 h_{2001}-i\omega_2 h_{2001}-C(\tau;v_1,v_1,\bar v_2)\\
-B(\tau;\bar v_2,h_{2000})-2B(\tau;v_1,h_{1001})& = & 0,\ \tau \in [0,T], \\
h_{2001}(T)- h_{2001}(0) & = & 0,
\end{array}\right.
\end{equation}
\begin{equation}  \label{eq:BVP_h1020_NSNS}
\left\{\begin{array}{rcl}
 \dot h_{1020}-A(\tau) h_{1020}+i\omega_1 h_{1020}+2i\omega_2 h_{1020}\\
-C(\tau;v_1,v_2,v_2)-B(\tau;v_1,h_{0020})-2B(\tau;v_2,h_{1010})& = & 0,\ \tau \in [0,T], \\
h_{1020}(T)- h_{1020}(0) & = & 0,
\end{array}\right.
\end{equation}
and
\begin{equation}  \label{eq:BVP_h0120_NSNS}
\left\{\begin{array}{rcl}
 \dot h_{0120}-A(\tau) h_{0120}-i\omega_1 h_{0120}+2i\omega_2 h_{0120}\\
-C(\tau;\bar v_1,v_2,v_2)-B(\tau;\bar v_1,h_{0020})-2B(\tau;v_2,h_{0110})& = & 0,\ \tau \in [0,T], \\
h_{0120}(T)- h_{0120}(0) & = & 0.
\end{array}\right.
\end{equation}

The $\xi_2\left|\xi_2\right|^2$-terms from the homological equation make it possible to compute $b_{0021}$. Indeed, the differential equation
\begin{eqnarray*}
 \dot h_{0021}-A(\tau) h_{0021}+i\omega_2 h_{0021}&=&C(\tau;v_2,v_2,\bar v_2)+B(\tau;\bar v_2,h_{0020})+2B(\tau;v_2,h_{0011})\nonumber\\
&& -2b_{0021}v_2-2\alpha_{0011}\dot v_2-2i\omega_2\alpha_{0011}v_2 \nonumber\\\label{eq:h0021_NSNS}
\end{eqnarray*}
results in a solvability
condition with $v_2^*$, i.e.
\begin{eqnarray*}
 \int_0^{T} \langle v_2^*,C(\tau;v_2,v_2,\bar v_2)+B(\tau;\bar v_2,h_{0020})+2B(\tau;v_2,h_{0011})\\
 -2b_{0021}v_2-2\alpha_{0011}\dot v_2-2i\omega_2\alpha_{0011}v_2 \rangle\; d \tau &=&0.
 \end{eqnarray*}
Therefore, considering the normalization condition from \eqref{eq:AdjEigenFunc_NSNS_3} and the differential equation from \eqref{eq:EigenFunc_NSNS_2}, we can calculate parameter $b_{0021}$
\begin{equation} \label{eq:b0021_NSNS}
 \boxed{b_{0021}=\frac{1}{2} \int_0^{T} \langle v_2^*,C(\tau;v_2,v_2,\bar v_2)+B(\tau;\bar v_2,h_{0020})+2B(\tau;v_2,h_{0011})\\
 -2\alpha_{0011}A(\tau) v_2 \rangle\; d \tau,}
\end{equation}
with $h_{0021}$ as the unique solution of the BVP
\begin{equation}  \label{eq:BVP_h0021_NSNS}
\left\{\begin{array}{rcl}
\dot h_{0021}-A(\tau) h_{0021}+i\omega_2 h_{0021}-C(\tau;v_2,v_2,\bar v_2)\\
-B(\tau;\bar v_2,h_{0020})-2B(\tau;v_2,h_{0011})\\
+2b_{0021}v_2+2\alpha_{0011}A(\tau) v_2& = & 0,\ \tau \in [0,T], \\
h_{0021}(T)- h_{0021}(0) & = & 0,\\
\int_0^{T} \langle v_2^*,h_{0021}\rangle \; d\tau & = & 0.
\end{array}
\right.
\end{equation}

The last two third order terms which we have to examine give us both the formula for a normal form coefficient. The first one, obtained from the $\left|\xi_1\right|^2\xi_2$-terms, gives us the BVP
\begin{equation}  \label{eq:BVP_h1110_NSNS}
\left\{\begin{array}{rcl}
\dot h_{1110}-A(\tau) h_{1110}+i\omega_2 h_{1110}-C(\tau;v_1,\bar v_1,v_2)-B(\tau;v_1,h_{0110})&&\\
-B(\tau;\bar v_1,h_{1010})-B(\tau;v_2,h_{1100})\\
+b_{1110}v_2+\alpha_{1100}A(\tau) v_2& = & 0,\ \tau \in [0,T], \\
h_{1110}(T)- h_{1110}(0) & = & 0,\\
\int_0^{T} \langle v_2^*,h_{1110}\rangle \; d\tau & = & 0,
\end{array}
\right.
\end{equation}
where from the solvability condition it follows that 
\begin{equation}\label{eq:b1110_NSNS}
 \boxed{b_{1110}=\int_0^{T} \langle v_2^*,C(\tau;v_1,\bar v_1,v_2)+B(\tau;v_1,h_{0110})+B(\tau;\bar v_1,h_{1010})+B(\tau;v_2,h_{1100}) \nonumber \\
-\alpha_{1100}A(\tau)v_2  \rangle\; d \tau.} 
\end{equation}
Analogously, we obtain the BVP
\begin{equation}  \label{eq:BVP_h1011_NSNS}
\left\{\begin{array}{rcl}
\dot h_{1011}-A(\tau) h_{1011}+i\omega_1 h_{1011}-C(\tau;v_1,v_2,\bar v_2)-B(\tau;v_1,h_{0011})\\
-B(\tau;v_2,h_{1001})-B(\tau;\bar v_2,h_{1010})+a_{1011}v_1+\alpha_{0011}A(\tau) v_1& = & 0,\ \tau \in [0,T], \\
h_{1011}(T)- h_{1011}(0) & = & 0,\\
\int_0^{T} \langle v_1^*,h_{1011}\rangle \; d\tau & = & 0,
\end{array}
\right.
\end{equation}
with 
\begin{equation} 
 \boxed{a_{1011}=\int_0^{T} \langle v_1^*,C(\tau;v_1,v_2,\bar v_2)+B(\tau;v_1,h_{0011})+B(\tau;v_2,h_{1001})+B(\tau;\bar v_2,h_{1010}) \nonumber \\
-\alpha_{0011}A(\tau)v_1  \rangle\; d \tau. } \label{eq:a1011_NSNS}
\end{equation}
We still need the coefficients $b_{1101}$ and $a_{0111}$ which are determined by 
\begin{eqnarray}
 b_{1101}=\int_0^{T} \langle \bar v_2^*,C(\tau;v_1,\bar v_1,\bar v_2)+B(\tau;v_1,h_{0101})+B(\tau;\bar v_1,h_{1001})+B(\tau;\bar v_2,h_{1100}) \nonumber \\
-\alpha_{1100}A(\tau)\bar v_2  \rangle\; d \tau && 
\end{eqnarray}
and
\begin{eqnarray}
 a_{0111}=\int_0^{T} \langle \bar v_1^*,C(\tau;\bar v_1,v_2,\bar v_2)+B(\tau;\bar v_1,h_{0011})+B(\tau;v_2,h_{0101})+B(\tau;\bar v_2,h_{0110}) \nonumber\\
-\alpha_{0011}A(\tau)\bar v_1  \rangle\; d \tau. &&
\end{eqnarray}

As before, the higher order terms which determine the stability of the torus can be found in Appendix C in \cite{lc2nf_arxiv}.


\subsection{Implementation}\label{Section:Implementation}
Numerical implementation of the formulas derived in the previous section requires the evaluation of 
integrals of scalar functions over $[0,T]$ and the solution of nonsingular linear BVPs with integral 
constraints. Such tasks can be carried out within the standard continuation software such as {\sc auto} 
\cite{AUTO97}, {\sc content} \cite{CONTENT}, and {\sc matcont} \cite{MATCONT}. In these software packages, 
periodic solutions to (\ref{ODE}) are computed with the method of {\em orthogonal collocation} with 
piecewise polynomials applied to properly formulated BVPs \cite{BoSw:73,BVPbook:95}. 

We have implemented our algorithms in {\sc matcont} analogously to the eight cases with $n_c\leq3$. For 
further details we refer to \cite{drdwgk} where this is extensively discussed.


==> normalforms.tex <==
\section{Normal forms on the center manifold and their bifurcations}
\label{Section:Normalforms}
Write (\ref{ODE}) at the critical parameter values as
%
\begin{equation}\label{eq:P.1}
\dot{u}=F(u)
\end{equation}
%
and suppose that there is a limit cycle $\Gamma$ corresponding to a
periodic solution $u_0(t)=u_0(t+T)$, where $T>0$ is its (minimal)
period. Expand $F(u_0(t)+v)$ into the Taylor series
%
\begin{equation} \label{eq:MULT}
\begin{array}{rcl}
F(u_0(t)+v) &=& F(u_0(t)) + \\
&&A(t)v + {\displaystyle \frac{1}{2}B(t;v,v) + \frac{1}{3!}C(t;v,v,v)} + \\
&&{\displaystyle\frac{1}{4!}D(t;v,v,v,v) +
\frac{1}{5!}E(t;v,v,v,v,v) + O(\|v\|^6)},
\end{array}
\end{equation}
%
where $A(t)=F_u(u_0(t))$ and
$$
B(t;v_1,v_2)=F_{uu}(u_0(t))[v_1,v_2],~~
C(t;v_1,v_2,v_3)=F_{uuu}(u_0(t))[v_1,v_2,v_3],
$$
etc. The matrix $A$ and the multilinear forms $B,C,D,$ and $E$ are periodic in $t$
with period $T$ but this dependence will often not be indicated
explicitly.
\par
Consider the initial-value problem for the fundamental matrix
solution $Y(t)$, namely,
%
\begin{equation*} \label{P.2}
\frac{dY}{dt}=A(t)Y,\ \ Y(0)=I_n,
\end{equation*}
%f
where $I_n$ is the $n\times n$ identity matrix. The eigenvalues of
the monodromy matrix $M=Y(T)$ are called ({\em Floquet}) {\em
multipliers} of the limit cycle. The multipliers with $|\mu|=1$ are
called {\em critical}. There is always a ``trivial" critical
multiplier $\mu_n=1$. We denote the total number of critical
multipliers by $n_c$ and assume that the limit cycle is
non-hyperbolic, i.e. $n_c > 1$. In this case, there exists an
invariant $n_c$-dimensional {\em critical center manifold}
$W^c(\Gamma) \subset {\mathbb R}^n$ near $\Gamma$\footnote{This
manifold should not be confused with the $(n_c-1)$-dimensional center
manifold of the corresponding Poincar\'{e} map.}.


\subsection{Critical normal forms}
It is well known \cite{Ar:83,Ku:2004} that in generic
two-parameter systems (\ref{ODE}) only eleven codim 2 local bifurcations
of limit cycles occur. To describe the normal forms of (\ref{eq:P.1}) on the
critical center manifold $W^c(\Gamma)$ for these codim 2 cases, we
parameterize  $W^c(\Gamma)$ near $\Gamma$ by $(n_c-1)$ transverse coordinates and 
$\tau \in [0,kT]$ for $k \in \{1,2,3,4\}$, depending on the bifurcation. The $8$ cases 
where $n_c\leq 3$ were treated in \cite{drdwgk}. Based on \cite{Io:88} we show 
in Appendix A in \cite{lc2nf_arxiv} that the restriction of (\ref{eq:P.1}) to the
corresponding critical center manifold $W^c(\Gamma)$ with $n_c=4$ or $n_c=5$ will 
take one of the following {\it Iooss normal forms}. 

\subsubsection{LPNS}
The {\em Limit Point -- Neimark-Sacker} bifurcation occurs when the
trivial critical multiplier $\mu_n=1$ corresponds to a two-dimensional Jordan block and there are only
two more critical simple multipliers $\mu_{1,2}=e^{\pm i\theta}$
with $\theta\neq \frac{2 \pi}{j}$, for $j=1,2,3,4$. The four-dimensional Iooss normal form at the LPNS 
bifurcation is derived in Appendix A.1.1 in \cite{lc2nf_arxiv} and can be written as
\begin{equation} \label{eq:NF-LPNS}
\begin{cases}
 \ds\dd{\tau}{t}=1-\xi_1+\alpha_{200} \xi_1^2+\alpha_{011}\left|\xi_2\right|^2+\alpha_{300} \xi_1^3+\alpha_{111} \xi_1\left|\xi_2\right|^2+\ldots, \smallskip \\
 \ds\dd{\xi_1}{\tau}= a_{200} \xi_1^2+a_{011}\left|\xi_2\right|^2+a_{300} \xi_1^3+a_{111} \xi_1\left|\xi_2\right|^2+\ldots, \smallskip \\
 \ds\dd{\xi_2}{\tau}= i\omega \xi_2+b_{110} \xi_1\xi_2+b_{210} \xi_1^2 \xi_2+b_{021} \xi_2\left|\xi_2\right|^2 +\ldots, \smallskip\\
\end{cases}
\end{equation}
where $\tau \in [0,T]$, $\omega = \theta/T$, $\xi_1$ is a real coordinate and $\xi_2$ is a complex
coordinate on $W^c(\Gamma)$ transverse to $\Gamma$, $\alpha_{ijk},a_{ijk}\in \R, b_{ijk} \in \C$, and 
the dots denote the $O(\|\xi^4\|)$-terms, which are $T$-periodic in $\tau$. The equations (\ref{eq:NF-LPNS}) 
implicitly describe motions on the $4$-dimensional invariant manifold $W^c(\Gamma)$ with one cyclic 
coordinate $\tau$.

\subsubsection{PDNS}
The {\em Period-Doubling -- Neimark-Sacker} bifurcation occurs when the
trivial critical multiplier $\mu_n=1$ is simple and there are only
three more critical simple multipliers, namely $-1$ and $\mu_{1,2}=e^{\pm i\theta}$
with $\theta\neq \frac{2 \pi}{j}$, for $j=1,2,3,4$. The four-dimensional Iooss normal form at the PDNS 
bifurcation is derived in Appendix A.1.2 in \cite{lc2nf_arxiv} and can be written as
\begin{equation} \label{eq:NF-PDNS}
\begin{cases}
 \ds\dd{\tau}{t}=1+\alpha_{200} \xi_1^2+\alpha_{011}\left|\xi_2\right|^2+\alpha_{400} \xi_1^4+\alpha_{022}\left|\xi_2\right|^4+\alpha_{211} \xi_1^2\left|\xi_2\right|^2+\ldots, \smallskip \\
 \ds\dd{\xi_1}{\tau}= a_{300} \xi_1^3+a_{111}\xi_1\left|\xi_2\right|^2+a_{500} \xi_1^5+a_{122} \xi_1\left|\xi_2\right|^4+a_{311} \xi_1^3\left|\xi_2\right|^2+\ldots, \smallskip \\
 \ds\dd{\xi_2}{\tau}= i\omega \xi_2+b_{210} \xi_1^2\xi_2+b_{021} \xi_2\left|\xi_2\right|^2+b_{410} \xi_1^4\xi_2+b_{221} \xi_1^2\xi_2\left|\xi_2\right|^2+b_{032} \xi_2\left|\xi_2\right|^4+\ldots, \smallskip\\
\end{cases}
\end{equation}
where $\tau \in [0,2T]$, $\omega = \theta/T$, $\xi_1$ is a real coordinate and $\xi_2$ is a complex
coordinate on $W^c(\Gamma)$ transverse to $\Gamma$, $\alpha_{ijk},a_{ijk}\in \R, b_{ijk} \in \C$, and 
the dots denote the $O(\|\xi^6\|)$-terms, which are $2T$-periodic in $\tau$. The equations 
(\ref{eq:NF-PDNS}) implicitly describe motions on the $4$-dimensional invariant manifold $W^c(\Gamma)$ that is 
doubly covered by the selected coordinates.

\subsubsection{NSNS}
The {\em double Neimark-Sacker} bifurcation occurs when the
trivial critical multiplier $\mu_n=1$ is simple and there are only
four more critical simple multipliers $\mu_{1,4}=e^{\pm i\theta_1}$ and $\mu_{2,3}=e^{\pm i\theta_2}$
with $\theta_{1,2}\neq \frac{2 \pi}{j}$, for $j=1,2,3,4,5,6$ and $l\theta_1 \neq j 
\theta_2$ for $l,j\in \mathbb{Z}$ with $l+j \leq 4$ (see \cite{GoGhKuMe:07}). 
The five-dimensional periodic normal form at the  NSNS bifurcation is derived 
in Appendix A.1.3 in \cite{lc2nf_arxiv} and can be written as
\begin{equation} \label{eq:NF-NSNS}
\left\{\begin{array}{rcl} \ds\dd{\tau}{t}&=&1+\alpha_{1100}\left|\xi_1\right|^2+\alpha_{0011}\left|\xi_2\right|^2\\
&&+\alpha_{2200}\left|\xi_1\right|^4+\alpha_{0022} \left|\xi_2\right|^4+\alpha_{1111} \left|\xi_1\right|^2\left|\xi_2\right|^2+\ldots, \\
 \ds\dd{\xi_1}{\tau}&=&i\omega_1 \xi_1 + a_{2100} \xi_1\left|\xi_1\right|^2+a_{1011}\xi_1\left|\xi_2\right|^2\\
 && + a_{3200}\xi_1\left|\xi_1\right|^4+a_{1022}\xi_1\left|\xi_2\right|^4+a_{2111}\xi_1\left|\xi_1\right|^2\left|\xi_2\right|^2+\ldots, \\
 \ds\dd{\xi_2}{\tau}&=& i\omega_2 \xi_2 + b_{0021} \xi_2\left|\xi_2\right|^2+b_{1110}\xi_2\left|\xi_1\right|^2\\
 && +b_{0032}\xi_2\left|\xi_2\right|^4+b_{2210}\xi_2\left|\xi_1\right|^4 +b_{1121}\xi_2\left|\xi_1\right|^2\left|\xi_2\right|^2+\ldots, \\
\end{array}
\right.
\end{equation}
where $\tau \in [0,T]$, $\omega_{1,2} = \theta_{1,2}/T$, $\xi_1$ and $\xi_2$ are complex
coordinates on $W^c(\Gamma)$ transverse to $\Gamma$, $\alpha_{ijkl}\in \R,a_{ijkl},b_{ijkl} \in \C$, 
and the dots denote the $O(\|\xi^6\|)$-terms, which are $T$-periodic in $\tau$. The equations 
(\ref{eq:NF-NSNS}) implicitly describe motions on a $5$-dimensional manifold with one cyclic 
coordinate $\tau$.

\subsection{Generic unfoldings of the critical normal forms}
\label{Appendix:2}
Here we describe how the coefficients of the critical normal forms can be used to predict
bifurcations of the phase portraits near the critical limit cycles for nearby parameter values.
We introduce certain quantities -- computable in terms of these coeffcients -- that are reported in 
the {\sc matcont} output and used to distinguish between various bifurcation scenarios in examples
in Section \ref{Section:Examples}. 

In generic two-parameter systems (\ref{ODE}) the considered bifurcations occur at isolated parameter values.
By translating the origin of the parameter plane to one of such points, we can consider an {\em unfolding}
of the corresponding bifurcation and study its canonical local bifurcation diagram for nearby parameter values.
It is well known that the critical center manifold $W^c(\Gamma)$ can be smoothly continued w.r.t. $p$ 
in a neighborhood of the bifurcation point, so that the restriction of (\ref{ODE}) to this manifold can 
be studied. Choosing appropriate coordinates $(\xi,\tau)$ on this parameter-dependent invariant manifold, 
one can transform the restricted system into a parameter-dependent normal form in which 
$\frac{d\xi}{d\tau}$ has a $\tau$-independent principle part and higher-order
terms which are $kT$-periodic in $\tau$ with $k=1$ for LPNS and NSNS and $k=2$ for PDNS.
Below we describe bifurcations of these principle parts, i.e., the truncated parameter-dependent
autonomous normal forms. Since the dynamics is determined by the $\xi$-equations, we first focus on 
their bifurcations and then interpret appearing bifurcation diagrams for the original system (\ref{ODE}). 
The new unfolding parameters will be denoted by $(\beta_1,\beta_2)$. 


\subsubsection{LPNS}\label{Appendix:2LPNS}
Generically, a two-parameter unfolding of (\ref{ODE}) near this bifurcation restricted to the center manifold
is smoothly orbitally equivalent (with possible time reversal) to a system in which the equations for 
the transverse coordinates have the form
\begin{equation}
\label{lpnsnormalform}
\left\{\begin{array}{rcl}
 {\displaystyle \frac{d\xi}{d\tau}} &=& \beta_1 + \xi^2+ s \left|\zeta\right|^2 +
 O(\|(\xi,\zeta,\bar{\zeta})\|^4), \vspace{0.2cm}\\ 
 {\displaystyle \frac{d\zeta}{d\tau}} &=&  (\beta_2+i\omega_1)\zeta + 
 (\theta +i\vartheta)\xi \zeta+\xi^2\zeta + O(\|(\xi,\zeta,\bar{\zeta})\|^4),
 \end{array}\right.
\end{equation}
where the $O$-terms are still $T$-periodic in $\tau$. This system is similar to the
normal form for the Zero-Hopf bifurcation of equilibria (cf. Theorem 8.6 on page 338 in \cite{Ku:2004}). 
In Figure \ref{fig:NF_LPNS} the four possible bifurcation diagrams of the amplitude system 
for (\ref{lpnsnormalform}) without the $O$-terms,
\begin{equation}
\label{lpnsamplitude}
\left\{\begin{array}{rcl}
\dot{\xi}&=& \beta_1 + \xi^2 + s \rho^2,\\
\dot{\rho} &=& \rho (\beta_2 + \theta \xi + \xi^2),
\end{array}
\right.
\end{equation}
are reported depending on the sign of the normal form coefficients $s$ and $\theta$ \cite{Ku:2004}. 
Here and in what follows a dot means the derivative w.r.t. $\tau$.
\begin{figure}[htb]
\centering
 \subfigure[$s=1, \theta>0$]{
 \includegraphics[width=.48\textwidth]{images/LPNS1}\label{fig:NF_LPNS_1}}\subfigure[$s=-1, \theta<0$]{
 \includegraphics[width=.48\textwidth]{images/LPNS2}}
 \subfigure[$s=1, \theta<0$]{
 \includegraphics[width=.48\textwidth]{images/LPNS3}}\subfigure[$s=-1, \theta>0$]{
 \includegraphics[width=.48\textwidth]{images/LPNS4}}
 \caption{Bifurcation diagrams of the truncated amplitude system (\ref{lpnsamplitude}) for the LPNS bifurcation.} 
\label{fig:NF_LPNS}
\end{figure}
\par
Let us now discuss the interpretation of the phase portraits in the $(\xi,\rho)$-plane of the truncated 
amplitude system in the context of the bifurcating limit cycle. The fixed points or limit cycles have additional dimensions from 
the phases of the periodic orbit itself plus the phases ignored in the reduction to the amplitude 
system. We note that in the amplitude system the vertical direction always corresponds to a 
Neimark-Sacker bifurcation, but that the horizontal component of the phase space has a different 
meaning. For LPNS, equilibria on the horizontal axis correspond to limit cycles. Equilibria
off the horizontal axis correspond to invariant 2D tori $\mathbb{T}^{2}$ and the periodic 
orbit which exists if $s\theta<0$ corresponds to an invariant 3D torus $\mathbb{T}^{3}$. 
\par
The critical values of $s$ and $\theta$ can be expressed in terms of the coeffcients of 
(\ref{eq:NF-LPNS}) as
$$
s=\mbox{sign }(a_{200}a_{011}),~~\theta = \frac{\Re(b_{110})}{a_{200}}.
$$ 
These values determine the bifurcation scenario. For $s\theta<0$, a $3$-torus appears in the unfolding via a Neimark-Sacker
bifurcation. The stability of 
this torus is determined by the third order terms in (\ref{eq:NF-LPNS}). Indeed, the sign of the 
corresponding first Lyapunov coefficient for the Hopf bifurcation in (\ref{lpnsamplitude}) is opposite to 
that of $\theta$ but the `time' in  (\ref{lpnsnormalform}) is rescaled with factor
$$
E = \Re\left(b_{210}+b_{110}\left( \frac{\Re(b_{021})}{a_{011}} - \frac{3a_{300}}{2a_{200}}+ 
\frac{a_{111}}{2a_{011}}\right)- \frac{b_{021}a_{200}}{a_{011}}\right).
$$
(see page 337 in \cite{Ku:2004}). If $E \cdot l_1<0$, an unstable $3$-torus appears, 
if $E \cdot l_1>0$, the $3$-torus is stable. The output given by {\sc matcont} is $(s,\theta,E)$ 
\footnote{Remark that $E=NaN$ is reported when terms up to only the second order are computed.}.
\par

Note that Figure \ref{fig:NF_LPNS} presents  bifurcations of 
the truncated system (\ref{lpnsnormalform}) that only {\em approximates} the full normalized unfolding. 
In particular, the orbit structure on the invariant tori can differ from that
for the approximating system due to phase locking. Moreover,  the destruction of $\mathbb{T}^{3}$ via a 
heteroclinic bifurcation in case (c) of Figure \ref{fig:NF_LPNS} becomes a complicated sequence of global bifurcations involving 
stable and unstable invariant sets of cycles and tori. All these bifurcations, however, occur in the
exponentially-small parameter wedge near the heteroclinic bifurcation curve $P$. For detailed discussions
of the effects of the truncation, also in the two other cases, we refer to \cite{KuMe:2006,BSV:2010} and references therein.


\subsubsection{PDNS} \label{Appendix:2PDNS}
Generically, a two-parameter unfolding of (\ref{ODE}) near this bifurcation restricted to the center manifold
is smoothly orbitally equivalent to a system in which the equations for 
the transverse coordinates have the form
\begin{equation}
\left\{ 
\begin{array}{rcl}
\dot v_1 &=&\mu_1v_1+P_{11}v_1^3+P_{12}v_1\left|v_2\right|^2+S_1v_1\left|v_2\right|^4 + O(\|(v_1,v_2,\bar{v}_2)\|^6), \smallskip \\ 
\dot v_2 &=&(\mu_2+i\omega_2)v_2+P_{21}v_1^2v_2+P_{22}v_2\left|v_2\right|^2+S_2v_1^4v_2+
iR_2v_2\left|v_2\right|^4 + O(\|(v_1,v_2,\bar{v}_2)\|^6),
\end{array}
\right.
\label{pdnsnormalform}
\end{equation}
where the $O$-terms are still $T$-periodic in $\tau$. This system is similar to one of the normal forms
for the Hopf-Hopf bifurcations of equilibria (cf. Lemma 8.14 on page 354 in \cite{Ku:2004}).

The amplitude system for (\ref{pdnsnormalform}) without the $O$-terms is
\begin{equation}
\label{pdnsamplitude}
\left\{\begin{array}{rcl}
\dot{r}_1 &=& r_1(\mu_1 + p_{11}r_1^2 + p_{12}r_2^2 + s_1 r_2^4),\\
\dot{r}_2 &=& r_1(\mu_2 + p_{21}r_1^2 + p_{22}r_2^2 + s_2 r_1^4),
\end{array}
\right.
\end{equation}
where
$$
p_{11} = P_{11},~  p_{12} = P_{12},~  p_{21} = \Re(P_{21}),~  p_{22} = \Re(P_{22}),~  s_1 = S_{1},~  s_2 = \Re(S_{2}).
$$
The values of $p_{jk}$ and $s_j$, for $j,k=1,2$, and the quantities
\begin{eqnarray*}
\theta = \frac{p_{12}}{p_{22}}, \delta = \frac{p_{21}}{p_{11}}, 
\Theta = \frac{s_1}{p_{22}^2}, \Delta = \frac{s_2}{p_{11}^2}
\label{bifanalysispdns1}
\end{eqnarray*}
indicate in which bifurcation scenario we are (see Section 8.6.2 in \cite{Ku:2004}). 
\par
In the ``simple" case where $p_{11}p_{22}>0$, there are five topologically different bifurcation diagrams
of the truncated amplitude system (\ref{pdnsamplitude}), corresponding to the following cases: 
\begin{itemize}
	\item[I.] $\theta>0, \delta>0, \theta\delta>1$
	\item[II.] $\theta>0, \delta>0, \theta\delta<1$
	\item[III.] $\theta>0, \delta<0$
	\item[IV.] $\theta<0, \delta<0, \theta\delta<1$
	\item[V.] $\theta<0, \delta<0, \theta\delta>1$	
\end{itemize}
If $\delta >\theta$, reverse the role of $\theta$ and $\delta$. Each case corresponds with a 
region in the $(\theta,\delta)$-plane, see Figure \ref{fig:NF_PDNSoverview} (a). The 
parametric portraits belonging to the different regions can be seen in Figure \ref{fig:NF_PDNSsimple} (a), 
with corresponding phase portraits in the $(r_1,r_2)$-plane in Figure \ref{fig:NF_PDNSsimple} (b). 
The phase portraits are only shown for the case when $p_{11}<0$ and $p_{22}<0$. The case 
$p_{11}>0$ and $p_{22}>0$ can be reduced to the considered one by reversing time.

In the ``difficult" case where $p_{11}p_{22}<0$ however, there are six essentially different bifurcation 
diagrams: 
\begin{itemize}
	\item[I.] $\theta>1, \delta>1$
	\item[II.] $\theta>1, \delta<1, \theta\delta>1$
	\item[III.] $\theta>0, \delta>0, \theta\delta<1$
	\item[IV.] $\theta>0, \delta<0$
	\item[V.] $\theta<0, \delta<0, \theta\delta<1$	
	\item[VI.] $\theta<0, \delta<0, \theta\delta>1$	
\end{itemize}
The regions in the $(\theta,\delta)$-plane are shown in Figure \ref{fig:NF_PDNSoverview} (b). 
The related parametric portraits and phase portraits of (\ref{pdnsamplitude}) 
are given in Figure \ref{fig:NF_PDNSdifficult}.
Only the case $p_{11}>0$ and $p_{22}<0$ is presented, to which the opposite one can be easily reduced.

We note that Section 8.6.2 in \cite{Ku:2004} for the ``difficult" case contains
a few errors in the figures and in the asymptotic expression for the heteroclinic 
bifurcation curve\footnote{Unfortunately, there is also a minor misprint in our earlier ``correction" 
for the heteroclinic curve given in \cite{KuMe:2006}.}. Therefore, for completeness, we provide the figures
and correct asymptotics in \ref{Appendix:6}. 


\begin{figure}[htb]
\centering \subfigure[]{
 \includegraphics[width=.44\textwidth]{images/PDNS_overviewsimplecase}
 \label{fig:NF_PDNSoverviewleft}}
 \subfigure[]{
 \includegraphics[width=.44\textwidth]{images/PDNS_overviewdifficultcase}}
 \caption{(a) the five subregions in the $(\theta,\delta)$-plane in the ``simple" case; 
 (b) the six subregions in the $(\theta,\delta)$-plane in the ``difficult" case.} 
 \label{fig:NF_PDNSoverview}
\end{figure}

\begin{figure}[htb]
\centering \subfigure[]{
 \includegraphics[width=.44\textwidth]{images/PDNS_simplecase}
 \label{fig:NF_PDNSsimple_1}} 
 \subfigure[]{
 \includegraphics[width=.44\textwidth]{images/PDNS_simplecasebif}
 \label{fig:NF_PDNSsimple_2}}
 \caption{Bifurcation diagrams of the amplitude system (\ref{pdnsamplitude}) for the PDNS and NSNS bifurcations: 
 (a) parametric portraits in the ``simple" case; (b) phase portraits in the ``simple" case.} 
\label{fig:NF_PDNSsimple}
\end{figure}

\begin{figure}[htb]
\centering \subfigure[]{
 \includegraphics[width=.48\textwidth]{images/PDNS_difficultcase}}
 \subfigure[]{
 \includegraphics[width=.48\textwidth]{images/PDNS_difficultcasebif}}
 \caption{Bifurcation diagrams of the amplitude system (\ref{pdnsamplitude}) for the PDNS and NSNS bifurcations: 
 (a) parametric portraits in the ``difficult" case; 
 (b) phase portraits in the ``difficult" case.} 
 \label{fig:NF_PDNSdifficult}
\end{figure}

The critical values of $P_{jk}$ and $S_j$ can be expressed in terms of the coefficients of 
(\ref{eq:NF-PDNS}) as
$$
P_{11}= a_{300},~ P_{12}=a_{111},~ \Re(P_{21})= \Re(b_{210}),~ \Re(P_{22}) = \Re(b_{021}),
$$
and
\begin{eqnarray*}
S_1 &=& a_{122} + a_{111}\left( \frac{\Re(b_{221})}{\Re(b_{210})}-2 \frac{\Re(b_{032})}{\Re(b_{021})} - 
\frac{a_{500}\Re(b_{021})}{a_{300}\Re(b_{210})} \right),\\
\Re(S_2) &=&\Re(b_{410}) + \Re(b_{210})\left( \frac{a_{311}}{a_{111}}-2 \frac{a_{500}}{a_{300}} - 
\frac{a_{300}\Re(b_{032})}{a_{111}\Re(b_{021})} \right).
\end{eqnarray*}
(see page 356 in \cite{Ku:2004}). 

The fifth-order terms in (\ref{eq:NF-PDNS}) determine the stability of 
the tori in the ``difficult" cases. In fact, the sign of the first Lyapunov coefficient for 
the Neimark-Sacker bifurcation is given by
\begin{equation}
\label{l_1}
\mbox{sign } l_1 = -\mbox{sign}\left(\theta(\theta(\theta-1)\Delta+\delta(\delta-1)\Theta) \right).
\end{equation}
The output of {\sc matcont} is $(p_{11},p_{22},\theta,\delta,\mbox{sign } l_1)$\footnote{Remark 
that $\mbox{sign } l_1=NaN$ is reported when terms up to only the third order are computed.}.

For PDNS we have an interpretation analogous to LPNS, but the invariant sets may be ``doubled''. 
The origin always corresponds the original limit cycle. Other fixed points on the horizontal axis represent 
the period-doubled limit 
cycles, while a fixed point on the vertical axis corresponds to a $\mathbb{T}^{2}$. 
Fixed points off the coordinate 
axes correspond to doubled tori $\mathbb{T}^{2}$ and periodic orbits correspond to $\mathbb{T}^{3}$.
As in the LPNS case, Figures \ref{fig:NF_PDNSsimple} and \ref{fig:NF_PDNSdifficult} present  
bifurcations of the truncated amplitude system that only {\em approximates} the 
full normalized unfolding. In particular, one has to be carefull with `torus doubling', which is in fact a complicated
quasiperiodic bifurcation \cite{Los:1989,ViBrSi:2011}.


\subsubsection{NSNS}\label{Appendix:2NSNS}
Generically, a two-parameter unfolding of (\ref{ODE}) near this bifurcation restricted to the center manifold
is smoothly orbitally equivalent to a system in which the equations for 
the transverse coordinates have the form
\begin{equation} 
\begin{cases}
\dot v_1 =(\mu_1+i\omega_1)v_1+P_{11}v_1\left|v_1\right|^2+P_{12}v_1\left|v_2\right|^2
+iR_1v_1\left|v_1\right|^4+S_1v_1\left|v_2\right|^4 + O(\|(v,\bar{v})\|^6), \\ 
\dot v_2 =(\mu_2+i\omega_2)v_2+P_{21}v_2\left|v_1\right|^2+P_{22}v_2\left|v_2\right|^2+
S_2v_2\left|v_1\right|^4+iR_2v_2\left|v_2\right|^4 + O(\|(v,\bar{v})\|^6),
\end{cases}
\label{nsnsnormalform}
\end{equation}
where the $O$-terms are $T$-periodic in $\tau$. Neglecting this periodicity, system (\ref{nsnsnormalform}) is the
normal form for the Hopf-Hopf bifurcation of equilibria (cf. Lemma 8.14 on page 354 in \cite{Ku:2004}).

The truncated amplitude system for (\ref{nsnsnormalform}) is the same as (\ref{pdnsamplitude}), where now
\begin{eqnarray*}
&&p_{11}=\Re(P_{11})= \Re(a_{2100}), ~p_{12}=\Re(P_{12})= \Re(a_{1011}),\\
&&p_{21}=\Re(P_{21})= \Re(b_{1110}), ~p_{22}=\Re(P_{22}) = \Re(b_{0021}),
\end{eqnarray*}
and 
\begin{eqnarray*}
&& s_1= \Re(S_1) = \Re(a_{1022}) + 
\Re(a_{1011})\left( \frac{\Re(b_{1121})}{\Re(b_{1110})}-2 
\frac{\Re(b_{0032})}{\Re(b_{0021})} - \frac{\Re(a_{3200})\Re(b_{0021})}{\Re(a_{2100})\Re(b_{1110})} \right),\\
&& s_2 = \Re(S_2) =\Re(b_{2210}) + 
\Re(b_{1110})\left( \frac{\Re(a_{2111})}{\Re(a_{1011})}-2 
\frac{\Re(a_{3200})}{\Re(a_{2100})} - \frac{\Re(a_{2100})\Re(b_{0032})}{\Re(a_{1011})\Re(b_{0021})} \right).
\end{eqnarray*}
The output of {\sc matcont} is $(p_{11},p_{22},\theta,\delta,\mbox{sign } l_1)$\footnote{Remark 
that $\mbox{sign } l_1=NaN$ is reported when terms up to only the third order are computed.}. 


Although the phase portraits of the truncated amplitude system are the same as for PDNS, 
their interpretation is slightly different, since they `live' in the $(|v_1|,|v_2|)$-plane. Here, on both axes the fixed points 
correspond to invariant 2D tori $\mathbb{T}^{2}$ 
for the original system. Fixed points off the coordinate axes and limit cycles correspond to $\mathbb{T}^{3}$ 
and $\mathbb{T}^{4}$, respectively. The usual remark on the approximate nature of the bifurcation diagrams
applies here as well.


